Causal Structural Learning Via Local Graphs

We consider the problem of learning causal structures in sparse high-dimensional settings that may be subject to the presence of (potentially many) unmeasured confounders, as well as selection bias. Based on the structure found in common families of large random networks and examining the representation of local structures in linear structural equation models (SEM), we propose a new local notion of sparsity for consistent structure learning in the presence of latent and selection variables, and develop a new version of the Fast Causal Inference (FCI) algorithm with reduced computational and sample complexity, which we refer to as local FCI (lFCI). The new notion of sparsity allows the presence of highly connected hub nodes, which are common in real-world networks, but problematic for existing methods. Our numerical experiments indicate that the lFCI algorithm achieves state-of-the-art performance across many classes of large random networks, and its performance is superior to that of existing methods for networks containing hub nodes.

==> proof_enumeration.tex <==
% \begin{figure}
% 		\centering
% 		\begin{subfigure}[b]{0.2\linewidth}
% 		\begin{tikzpicture}[> = stealth,shorten > = 1pt,auto,node distance = 1cm,semithick]
% 		\tikzstyle{every state}=[draw = black,thick,fill = white,minimum size = 4mm]
		
% 		\node[c1] (i) at(0,0) {};
%         \node[c1] (u) at(1,0) {};

% 		\draw[->] (i) -- (u);
% 		\end{tikzpicture}
% 		\end{subfigure}
% 		\begin{subfigure}[b]{0.2\linewidth}
% 		\begin{tikzpicture}[> = stealth,shorten > = 1pt,auto,node distance = 1cm,semithick]
% 		\tikzstyle{every state}=[draw = black,thick,fill = white,minimum size = 4mm]
		
% 		\node[c1] (i) at(0,0) {};
%         \node[c2] (u) at(1,0) {};

% 		\draw[->] (u) -- (i);
% 		\end{tikzpicture}
% 		\end{subfigure}
% 		\begin{subfigure}[b]{0.2\linewidth}
% 		\begin{tikzpicture}[> = stealth,shorten > = 1pt,auto,node distance = 1cm,semithick]
% 		\tikzstyle{every state}=[draw = black,thick,fill = white,minimum size = 4mm]
		
% 		\node[c1] (i) at(0,0) {};
%         \node[c1] (u) at(1,0) {};

% 		\draw[<->] (u) -- (i);
% 		\end{tikzpicture}
% 		\caption{Move}
% 		\end{subfigure}
% 		\caption{Enumeration}
% 	\end{figure}

==> trekdecomp.tex <==
In this section we provide an algebraic explanation of Assumption~\ref{ass:vanishtrekweight}. 
In particular, we review the trek representation of partial correlation in linear SEM.  The representation clarifies that conditional dependence in a linear SEM is tied to existence of paths/treks in the graph underlying the model.  This allows us to argue  that conditional dependence is typically induced by short versus long treks, which in turn provides the basis for exploiting small local separators in our algorithms. 

%In the previous section, we observed that many large random networks have small local separators. 
%To utilize this property when learning the structure of such networks, in 
%%can be well-represented by such graphs, using only short paths, these relations can be discovered %effectively via their local graph structures. 
%this section, we review the trek representation of partial correlation in 
%linear structural equation models (SEMs). Using this representation, we show that long treks have %vanishing contribution to partial correlation, and can thus be ignored when only conditioning on %small sets. 

%In Gaussian graphical models, conditional independence statements in the form of
%$X_A\independent X_B|X_C$ are characterized by rank dropping condition of the covariance matrix, namely, $\rank(\Sigma(A\cup C,B\cup C))\leq |C|$ 
%\cite[see, e.g.,][]{sullivant2018}. 
\subsection{Treks and $m$-separation}
This section relies on the 
\textit{trek representation}
\citep{wright1934,sullivant2010,draisma2013} of covariance matrix $\Sigma$.
To simplify the discussion, we present the following results assuming there is no
 selection variables in the graph, and therefore $G$ is a MAG without undirected edges. 
In a mixed graph $G$, we define a \textit{trek} from node $i$ to $j$ as a tuple $\tau=(P_L,P_M,P_R)$, 
where $P_L$ is a directed path from some node $s$ to $i$,
and $P_R$ is a directed path 
from some node $t$ to $j$,
%in the form of  $(t-\ldots-v\to \ldots \to j)$,
and $P_M$ is either one bidirected edge $s\edgeheadhead t$ (when $P_L$ and $P_R$ possesses no undirected edge) or the empty set when $s=t$. 
We call $i$ the \textit{initial node}, $j$ the \textit{final node}, and $s$ (or $\{s,t\}$) the \textit{top node(s)}.  
We define the 
\emph{trek monomial} as $m_\tau=\beta^L \omega_{s,t} \beta^R$, where $\beta^L=\prod_{k\to l\in P_L}\beta_{kl}$ and $\beta^R=\prod_{k\to l\in P_R}\beta_{kl}$, 
and 
let $\mathcal{T}(i,j)$ denote the set of all trek  from $i$ to $j$. 
Moreover, 
for sets $C$ and $D$ with $|C|=|D|=k$, we define
a \textit{trek system} $T$ from $C$ to $D$ as a set of $k$ treks whose initial nodes exhaust 
$C$ and final nodes exhaust $D$. 
With abuse of notation we write  $T$ as a tuple of collections of paths $(P_L,P_M,P_R)$.
We define the \textit{trek system monomial} as the product of  trek monomials in the system, i.e.,  $m_T=\prod_{\tau\in T}m_\tau$. 
% If we write $C=\{c_1,\ldots,c_k\}$ and $D=\{d_1,\ldots, d_k\}$, then
Each trek system determines a permutation of the initial and final nodes, and we define the the sign of this trek system as the
sign of the its permutation. 
 Let $\mathcal{T}(C,D)$ denote  the collection of all trek systems from $C$ to $D$.
By the Cauchy–Binet determinant expansion, we have,
 \begin{align}
 \det \Sigma(C,D)& =\sum_{R,S\subset V, |R|=|S|=k} \det\left((I-B)^{-\top}\right)_{C,R} \det\Omega_{R,S}\det \left((I-B)^{-1}\right)_{S,D} \\
 &= \sum_{T\in \mathcal{T}(C,D)}\sign(T)m_T.\label{eq:trekdecomp}
 \end{align} 

 

% An important property of linear SEMs is that the covariance between 
% $i$ and $j$ can be described by the 
% ``trek rule" \citep{wright1934,sullivant2010,draisma2013}:
% \begin{equation}\label{eq:trekrule}
% \Sigma(i,j) = \sum_{\tau\in\mathcal{T}(i,j)}m_\tau.
% \end{equation}


% Conditional independence relations among the variables can be characterized by
%  conditional covariance. 
% We write $\Sigma(C,D|S)$ as the covariance of $C$ and $D$ conditioned on $S$, and 
% $\Sigma(C,D)$ as the $(C,D)$ sub-matrix of 
% $\Sigma$. Using Schur complement, we get
% \begin{equation*}
% \Sigma(i,j|S)=\frac{\det(\Sigma(i\cup S, j\cup S))}{\det(\Sigma(S,S))}.
% \end{equation*} 



% The trek representation of the determinant terms is a
% generalization of  the trek rule \citep{sullivant2010}.
% For sets $C$ and $D$, with $|C|=|D|=k$, we define
% a \textit{trek system} $T$ from $C$ to $D$ as a set of $k$ treks whose initial nodes exhaust 
% $C$ and final nodes exhaust $D$. 
% We can write $T$ as a tuple $(P_L,P_M,P_R)$, where $P_L$ is a collection of $k$ directed paths from the top nodes of $T$ --- denoted $\TOP(T)$ --- to $C$, $P_R$ is a collection of $k$ directed paths from $\TOP(T)$ to $D$,  and $P_M$ is collection of single bidirected 
% edges in $\TOP(T)$.
% Similarly, 
% we define the \textit{trek system monomial} as the product of  trek monomials in the system, i.e.,  $m_T=\prod_{\tau\in T}m_\tau$. 
% If we write $C=\{c_1,\ldots,c_k\}$ and $D=\{d_1,\ldots, d_k\}$, then each 
%  trek system $T$ determines  a permutation $\pi$ such that the $k$ treks with 
%  initial nodes $\{c_1,\ldots,c_k\}$ has corresponding final nodes $\{d_{\pi(1)},\ldots,d_{\pi(k)}\}$. We denote the sign of the trek system, $\sign(T)$, as the sign of this permutation. 
%  Let $\mathcal{T}(C,D)$ denote  the collection of all trek systems from $C$ to $D$.
% By the Cauchy–Binet determinant expansion, we have,
%  \begin{align}
%  \det \Sigma(C,D)& =\sum_{R,S\subset V, |R|=|S|=k} \det((I-B)^{-\top})_{C,R} \det\Omega_{R,S}\det ((I-B)^{-1})_{S,D} \\
%  &= \sum_{T\in \mathcal{T}(C,D)}\sign(T)m_T.\label{eq:trekdecomp}
%  \end{align} 

 
We say a trek system $T$ has \textit{sided intersection} if two paths in $P_L$, $P_R$, or $P_M$ have shared nodes. 
% Let $T$ be a trek system from
% $i\cup S$ to $j\cup S$ for some
% set $S\subset V\setminus\{i,j\}$.
% Pasting together the paths in $T$ 
% we obtain a path $\pi(T)$ from $i$ to $j$. 
% If $T$ has no sided intersection, 
% then the path $\pi(T)$ is an 
% $m$-connecting path. 
% On the other hand, if $T$
% has sided intersections, 
% then $\pi(T)$ is blocked by $S$. 
If $T$ is a trek between $C$ and $D$ with sided intersections, then its trek system weight $m_T$ is cancelled in the summation in \eqref{eq:trekdecomp}, \citep[for a proof, see][]{sullivant2010}.
In other words, the summation in \eqref{eq:trekdecomp}
only needs to run over all trek systems without sided intersections.  
Consequently,  
$\det\left(\Sigma(i\cup S, j\cup S)\right)=0$
if and only if every system of treks from $i\cup S$ to $j\cup S$ has a sided intersection. 
The later condition is also called \textit{$t$-separation}. 
For Gaussian SEMs, in which conditional 
independence is characterized by 
zero partial correlation, this means
$W_i\independent W_j|W_S$ if and only if
$\sum_{T\in \mathcal{T}(i\cup S,j\cup S)}\sign(T)m_T=0$. 

%\subsection{Treks in local graphs}

% For SEMs that complies with the
% independence relations specified in 
% $\mathcal{I}(G)$, 
% conditional independence relations
% are characterized by partial 
% correlations, denoted as
% $\rho$. 
% Two nodes $i$ and $j$ 
% are non-adjacent in $G$ if and only if 
% there exists some $S\subset V\setminus \{i,j\}$ such that $\rho(i,j|S)=0$. 
% In PC and FCI,
% the output graph is inferred by
% hierarchical search for such 
% separator sets. 
% %This set $S$ is an exact, neighborhood-based $m$-separator. 
% We often observe in simulations that
% there might be some smaller set $S'\subset V\setminus \{i,j\}$ such that $\rho(i,j|S')$ is approximately zero. 
%For some fixed $\alpha>0$, we have $\{S:\rho(i,j|S)=0\}\subseteq \{S':|\rho(i,j|S')|<\alpha\}$, and therefore $\min_{S:|\rho(i,j|S')|<\alpha}\#S\leq \min_{S:\rho(i,j|S)=0} \# S$. 
%, and in their sample versions, decisions are made based by thresholding $\rho(i,j|S)$.
% In this case, 
% % not every trek system from $i\cup S'$ to $j\cup S'$ has sided intersection 
% % --- 
% % in other words, 
% there are a few $m$-connecting paths 
% between $i$ and $j$,
% % ---
% but their total weights are close to zero. 
% Such sets $S'$ are  approximate
% separators. 

%In PC and FCI, the graph structure is inferred by searching for a set $S$ for each node-pair $(i,j)$ such that $W_i\independent W_j|W_S$. 
%Such a separating set $S$ may be large in some cases, especially if we allow the maximum degree of $G$ to grow with $p$. 
%In contrast, we can often find some small set $S'$ such that $\Sigma(i,j|S')$ is approximately zero.
%Our next result indicates that under proper conditions, we can indeed learn independence relations from these small separators. 
% if only a small number of trek systems 
% between $i\cup S'$ and $j\cup S'$
% are without sided intersection, 
% and their trek system monomials vanishes
% with their total length, then 


% and their trek monomials vanishes 
% with their total lengths, 
% then 
% the  contribution of long $m$-connecting paths are ignorable in the trek representation of the determinant term. 

We will show next that Assumption~\ref{ass:vanishtrekweight} can be expressed
as a condition on trek weights. Let $G=(V,E)$ be a MAG. 
For non-adjacent nodes $i,j\in V$, and  
$S\subseteq V(G_\gamma)\setminus\{i,j\}$, 
we denote $\mathcal{T}_\gamma(i, j,S)$  as the collection of trek systems from $i\cup S$ to $j\cup S$ in $G_\gamma(i,j)$, and
$\mathcal{T}^C_\gamma(i , j, S) := \mathcal{T}(i , j, S) \setminus \mathcal{T}^C_\gamma(i , j, S) $. 
By our definition, $\mathcal{T}^C_\gamma(i , j, S) $ only contains treks with an edge not in $G_\gamma(i,j)$. 



\begin{lemma}\label{prop:trekdecomp}
Let $G=(V,E)$ be a MAG. Under Assumption~\ref{ass:cov}, 
 if 
 \[
 \max_{i\notin\ADJ(G,j)}\min_{S_\gamma\in \mathcal{S}_{\eta,\gamma}(i,j)}\left|\sum_{T\in \mathcal{T}^C_\gamma(i,j, S_\gamma)}\sign(T)m_T\right|=O(\beta^\gamma),
 \]
 where $\mathcal{S}_{\eta,\gamma}(i,j)$ is the collection of $\gamma$-local-graph separators of size at most $\eta$, 
 then Assumption~\ref{ass:vanishtrekweight} is satisfied. 
\end{lemma}
\begin{proof}
By Definition~\ref{def:localseparator}, if a set $S_\gamma$ is a $\gamma$-local-separator
of $(i,j)$, then it is a separator of $i$ and $j$ in $G_\gamma(i,j)$, so all 
trek systems between $i\cup S_\gamma$ and $j\cup S_\gamma$
have sided intersections in $G_\gamma(i,j)$, 
and hence also in $G$. 
Following \citet{sullivant2010} and \citet{draisma2013}, we only need to take summation over trek systems without sided intersection in $G$. 
Therefore, 
\begin{align*}
\sum_{T\in \mathcal{T}(i,j, S_\gamma)}\sign(T)m_T&=
\sum_{T\in \mathcal{T}_\gamma(i,j, S_\gamma)}\sign(T)m_T+\sum_{T\in \mathcal{T}^C_\gamma(i,j, S_\gamma)}\sign(T)m_T\\
&= \sum_{T\in \mathcal{T}^C_\gamma(i,j, S_\gamma)}\sign(T)m_T.
\end{align*}
Now denote $\Sigma(i,j|S_\gamma)$ as the $(i,j)$-th entry of the conditional variance matrix given $S_\gamma$. We have 
\begin{align*}
\rho(i,j|S_\gamma) &= \frac{\Sigma(i,j|S_\gamma)}{\sqrt{ \Sigma(i,i|S_\gamma)\Sigma(j,j|S_\gamma)  }}= \frac{\sum_{T\in \mathcal{T}(i,j, S_\gamma)}\sign(T)m_T}{\det(\Sigma(S_\gamma,S_\gamma))} \frac{1}{\sqrt{ \Sigma(i,i|S_\gamma)\Sigma(j,j|S_\gamma)  }}.
\end{align*}
By the fact that $\Sigma(j,j|S_\gamma) \geq \Sigma(j,j|V\setminus\{j\})\geq 1/\omega_{jj}$,
and $\det(\Sigma(S_\gamma,S_\gamma))\geq M^{-\eta}$ under Assumption~\ref{ass:cov}, we have $|\rho(i,j|S_\gamma)|=O(\beta^\gamma).$
\end{proof}

%%This lemma bridges the graphic and algebraic results. 
% In simulations, we observe that 
% for large enough $\gamma$, the covariance terms are usually well-characterized 
% by the treks in $\mathcal{T}_\gamma$. 
% 
%If contribution of long d-connecting paths are ignorable, 
%we could afford not 
% canceling them. 
%In other words, if $\sum_{T_\gamma\in \mathcal{T}^C(i\cup S,j\cup S)}\sign(T)m_T$ vanishes in 
%some order, say, $O(\beta^\gamma)$ for some $\beta<1$, then 
%under some faithfulness conditions, we can discover conditional independence relation
%by thresholding $\det \Sigma(i\cup S, j\cup S)$, or respectively, $\rho(i,j|S)$.  




%In practice, the data are often scaled such that each variable has
%unit standard deviation. In that case, $|\beta_{ij}|<1$ for most edges
%\citep{arjun2018} \textcolor{red}{most edges sounds mysterious, can we
%  be more precise, what is the effect of $\Omega$ not diagonal here?}. 





